Variational Tensor Network Simulation of Gaussian Boson Sampling and Beyond

The continuous variable quantum computing platform constitutes a promising candidate for realizing quantum advantage, as exemplified in Gaussian Boson Sampling. While noise in the experiments makes the computation attainable for classical simulations, it has been suggested that the addition of non-linear elements to the experiment will help retain the quantum advantage. We propose a classical simulation tool for general continuous variable sampling problems, including Gaussian Boson Sampling and beyond. We reformulate the sampling problem as that of finding the ground state of a simple few-body Hamiltonian. This allows us to employ powerful variational methods based on tensor networks and to read off the simulation error directly from the expectation value of the Hamiltonian. We validate our method by simulating Gaussian Boson Sampling, where we achieve results comparable to the state of the art. We also consider a non-Gaussian sampling problem, for which we develop novel local basis optimization techniques based on a non-linear parameterization of the implicit basis, resulting in high effective cutoffs with diminished computational overhead.

==> Sections/SM.tex <==
% \section{}
\subsection{
Effect of truncation on the spectrum of $\mathcal{H}$}
Equation 3 and 5 results in: $\text{spec}(\mathcal{H}) \in \{0,1,2,\hdots\}=\mathbbm{N}_0$. Therefore, the distribution of spectral weight for the variational state $|MPS\rangle$ can be alluded to by:
\begin{equation}
    \langle \mathcal{H}\rangle_{|MPS\rangle} = 0\cdot |c_0|^2 + \sum_{m=1}^\infty m|c_m|^2
\end{equation}
where $\sum_{m=0}|c_m|^2=1$ and $|c_0|^2$ is the object of interest. The $|c_m|^2$ is the total amplitude for all degenerate eigenvectors corresponding to the eigenvalue $m$ and, in principle, the $|c_m|^2$'s could be fitted by also considering higher moments $\langle \mathcal{H}^n\rangle$.

One could be concerned that once the projections are introduced and thus the spectrum altered, this will no longer be true. However, it can be shown (fig. \ref{appendix:figPerturbingTheEnergy}), that introducing the projections can only increase the eigenvalues \cite{Horn_Johnson_1985}. Furthermore, when they do increase, it is because the truncation $P$ introduced an error. Therefore, this metric remains trustworthy and a variational energy $\langle \mathcal{H}\rangle_{P|MPS\rangle}<1$ determines an acceptable simulation, depending on the wanted degree of accuracy. A larger variational energy could still result in an acceptable simulation, however, it would be harder to recognize.
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth, trim={0cm 3cm 7.4cm 11cm},clip]{new_figs/IncreaseInEnergy.pdf}
    \caption{\label{appendix:figPerturbingTheEnergy}Outline of how the energies of the truncated Hamiltonian is related to the original spectrum. $P_{\infty-1}$ is a projection onto a large enough Hilbert space such that the relevant part of the spectrum remain unaffected. The result of Cauchy's interlace theorem \cite{fbb19167-de4e-311f-b329-ce5946170d56} \cite{Horn_Johnson_1985} is that $\lambda_0 \leq\lambda_0'\leq\lambda_1\leq\lambda_1'\leq\hdots$ as exemplified by the brackets in the figure. The vertical lines are just one arbitrary manifestation and should not be taken too seriously (except for the $E_i$'s which truly are harmonic). The value of $\tilde{E}_0$ is investigated in fig. \ref{appendix:figTildeE0}.
    }
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{new_figs/PerturbationTheoryGSEnergy.pdf}
    \caption{To first order in perturbation theory $\Tilde{E}_0 \lesssim \langle \psi |P\mathcal{H}P|\psi\rangle$ (with $E_0=0$ and the inequality from numerical observation).
Indeed, the ground state energy forms a very nice line as a function of $\langle\mathcal{H}\rangle_{P|\psi\rangle}$}
\label{appendix:figTildeE0}
\end{figure}

\subsection{
Continuous Variable construction of $\mathcal{H}$}
Suppose we want to sample from a few-body wavefunction of the form:
\begin{equation}
    \psi(\pmb{x}) \propto e^{-\varphi(\pmb{x})}
\end{equation}
We can then define a generalized ladder operator:
\begin{equation}
    \hat{A}_k =\sum_l M^{-1/2}_{kl}\left(\hat{P}_l - i\frac{\partial\varphi(\pmb{x})}{\partial x_l}\bigg|_{\pmb{x}=\hat{\pmb{X}}}\right)
\end{equation}
or in vector notation:
\begin{equation}
\label{appendix:eqGeneralizedLoweringOp}
    \pmb{\hat{A}} = M^{-1/2}(\hat{\pmb{P}} - i\nabla\varphi(\hat{\pmb{X}})),
\end{equation}
where $\hat{\pmb{X}},\hat{\pmb{P}}$ are the canonical position and momentum operators. 
The positive semi-definite matrix $M$ is the mass-tensor. It is complimentary to the wavefunction and not given from experiment.
The generalized ladder operators eq. \ref{appendix:eqGeneralizedLoweringOp} are related to those found in super-symmetric quantum mechanics \cite{Drigo_Filho_2001}

If we set the mass matrix to be the identity:
\begin{equation}
    \hat{A}_k = \hat{P}_k - i\frac{\partial\varphi(\pmb{x})}{\partial x_k}\bigg|_{\pmb{x}=\hat{\pmb{X}}}
\end{equation}
then it is still true that $\pmb{\hat{A}}|\psi\rangle = 0$ and that $\pmb{\hat{A}}^\dagger\pmb{\hat{A}}$ is positive semi-definite.
However, with the introduction of a cutoff: $\hat{P} = \sum_k^{D-1}|\pmb{k}\rangle\langle\pmb{k}|$ we generally have, $\hat{P}\hat{A}_n\hat{P}|\psi\rangle = |\varphi_n\rangle$ where $|\varphi_n\rangle=0$, only when no truncation error is made from the projection.
Notice we still have positive semi-definiteness:
\begin{equation}
    \langle \pmb{\hat{A}}^\dagger\pmb{\hat{A}}\rangle_{P\psi} = \sum_n \langle \varphi_n|\varphi_n\rangle
\end{equation}
with each $\langle \varphi_n|\varphi_n\rangle\geq 0$. We can then consider the introduction of an arbitrary symmetric and positive-definite matrix, denoted the mass matrix $M$: 
\begin{equation}
\langle \pmb{\hat{A}}^\dagger\pmb{\hat{A}}\rangle_{P\psi} \rightarrow \langle \pmb{\hat{A}}^\dagger M^{-1}\pmb{\hat{A}}\rangle_{P\psi}
\end{equation}
such that
\begin{equation}
    \langle \pmb{\hat{A}}^\dagger M^{-1}\pmb{\hat{A}}\rangle_{P\psi} = 
    \sum_{nml} \langle \varphi_n|M^{-1/2}_{nl}M^{-1/2}_{lm}|\varphi_m\rangle =
    \sum_l \langle \Tilde{\varphi}_l|\Tilde{\varphi}_l\rangle
\end{equation}
which means that positive semi-definiteness is still obeyed but also that, once a truncation $P$ is introduced, the simulation can be affected by the choice of $M$. Furthermore, the choice of $M$ also has an effect on the commutation relations:
\begin{align}
    [\hat{A}_n,\hat{A}_m] &= 0\\
    [\hat{A}_n,\hat{A}^\dagger_m] &= 2M_{ni}^{-1/2}\text{Re}\left(\frac{\partial^2\varphi(\hat{\pmb{X}})}{\partial x_i\partial x_j}\right)M_{jm}^{-1/2}
\end{align}
such that if $\text{Re}(\varphi(\pmb{x}))$ is at most quadratic, $M$ can be chosen such that $[\hat{\pmb{A}},\hat{\pmb{A}}^\dagger] = \mathbbm{1}$. In the case of GBS and with this choice of $M$, a construction of $\mathcal{H}$ from eq. \ref{appendix:eqGeneralizedLoweringOp} yields exactly eq. 10.

Empirically (at least for GBS) the $M$ that make the generalized ladder operators obey the canonical commutation relations also improves the simulation, as opposed to choosing $M$ to be the identity.
In general however, numerics indicate that even though it provides an improvement, it will not be the optimal choice. The optimal choice remains elusive and it also seems to dependent on the specific choice of $D$.

\subsection{\label{appendix:MPSCompression}Compression to MPS form}
Imposing an MPS form on a state, with maximum bond dimension $\chi$, usually incurs an approximation error.
In order to define this error, first note that MPSs of a given bond dimension constitute a smooth manifold \cite{10.1063/1.4862851}
\begin{equation}
    \mathcal{M}_\chi = \{|\Phi\rangle : \text{MPS-rank}(|\Phi\rangle) = \chi\}
\end{equation}
$\text{MPS-rank}(|\Phi\rangle) = \chi$ means that $|\Phi\rangle$ can be decomposed as eq. 15 and 16 with the predefined bond dimension structure $\chi$.
By compression of a generic state $|\psi\rangle$ to its MPS form $|\psi_\text{MPS}\rangle$, we mean a retraction from the point generally outside the manifold onto the manifold \cite{SCHOLLWOCK201196}.
\begin{equation}
    |\psi_\text{MPS}\rangle = \underset{|\Phi\rangle \in \mathcal{M}_\chi}{\mathrm{argmin}}\big|\big||\psi\rangle - |\Phi\rangle\big|\big|^2
\end{equation}
There exist various approximations to $|\psi_\text{MPS}\rangle$ \cite{SCHOLLWOCK201196}\cite{PhysRevB.110.085149}. The one used in this paper relies on sequential singular value decompositions \cite{PhysRevLett.91.147902}\cite{Oh2024}. 
\begin{equation}
\label{eq:SVDApproximation}
   |\psi_\text{MPS}\rangle \approx \Tilde{|SVD\rangle}
   ,\quad
   |SVD\rangle = \frac{\Tilde{|SVD\rangle}}{\sqrt{\Tilde{\langle SVD}\Tilde{|SVD\rangle}}}
\end{equation}
hence the name "SVD" for the compressed state. The tilde is to indicate that the state generally will not be normalized and a subsequent renormalization is necessary.
Diagrammatically, if we denote a singular value decomposition by a dashed line, we may write:
\begin{equation}
\label{eq:SVDApproximationDiagram}
   \adjincludegraphics[valign=c,width=0.4\linewidth]{MPS_figs/SVDStateN5.png} \approx \adjincludegraphics[valign=c,width=0.4\linewidth]{MPS_figs/MPSN5.png}
\end{equation}
where the approximation is due to discarding all but the $\chi$ largest singular values. Note that the SVDs cannot be carried out simultaneously and it is this arbitrariness that demotes it from being an optimal rank $\chi$ compression.

Similarly to $\varepsilon_D$ we define:
\begin{equation}
\label{eq:epsilonchi}
   \varepsilon_\chi := \big|\big| |\psi\rangle - \Tilde{|SVD\rangle} \big|\big|^2
\end{equation}
which obeys the following bound \cite{OSELEDETS201070}\cite{doi:10.1137/090752286}\cite{doi:10.1137/S0895479896305696}:
\begin{equation}
\label{eq:QuasiOptimality}
    \varepsilon_\chi \leq \sum_{n=1}^{N-1} \sum_{k> \chi_i} \left(\sigma ^{(n)}_k\right)^2  \leq (N-1)\big|\big| |\psi\rangle - |\psi_\text{MPS}\rangle \big|\big|^2
\end{equation}
where $\sigma^{(n)}$ are the Schmidt coefficients when bipartitioning the state into $\{1,\hdots,n\}$ and $\{n+1,\hdots,N\}$. The fact that the compression by sequential SVDs is only quasi-optimal, is made manifest by the second inequality.
The first inequality can also be found in the physics literature \cite{PhysRevB.73.094423}\cite{PhysRevB.110.085149}\cite{RevModPhys.93.045003}\cite{PhysRevX.10.041038}.%Curiously, the first inequality is looser by a factor of two in the physics literature.
In practice, we circumvent the complications of the infinite dimensional Hilbert space in the definition of $\varepsilon_\chi$, by using the sum of squared singular values as a surrogate, eq. 26.

\subsection{\label{appendix:secTruncationErrorBound}Proof of $\varepsilon_D$ bound (eq. 40)}
Similar to eq. \ref{eq:QuasiOptimality}, the subsequent application of SVDs in the LBO procedure has its own quasi-optimality condition associated to it:
\begin{equation}
\label{eq:QuasiOptimality2}
    \big|\big||\psi\rangle - |\psi_\text{LBO}\rangle\big|\big|^2 \leq \sum_{i=1}^N \sum_{k> d_i} \left(\sigma ^{(i)}_k\right)^2 \leq N \big|\big||\psi\rangle - |\psi_\text{opt}\rangle\big|\big|^2
\end{equation}
where, now, $\sigma ^{(i)}_k$ are the eigenvalues of eq. 30, $|\psi_\text{LBO}\rangle$ is the physical state after truncation of the physical dimension in the optimal local basis and $|\psi_\text{opt}\rangle$ is the associated best rank $\{r_i\}$ approximation of the state $|\psi\rangle$.

However, the LBO based on the diagonalization of the reduced density matrices of the exact target state, is the optimal one \cite{PhysRevB.62.R747}, which means that:
\begin{equation}
\label{appendix:eqSVDOptimality}
    |\psi_\text{LBO}\rangle = P|\psi\rangle = |\psi_\text{opt}\rangle
\end{equation}
\\and the quasi-optimality condition eq. \ref{eq:QuasiOptimality2} becomes eq. 40 by the two observations:
\begin{align}
    |||\psi\rangle - P|\psi\rangle||^2
    &= 1 - \langle \psi | P |\psi \rangle = \varepsilon_D \\
    \quad \sum_{k=0}^\infty \left(\sigma_k^{(i)}\right)^2 &= 1
\end{align}
One way of seeing \ref{appendix:eqSVDOptimality} is to note that what made eq. \ref{eq:SVDApproximation} and eq. \ref{eq:SVDApproximationDiagram} approximate, is that each sequential SVD is affected by the one before it. When considering eq. 31 this is no longer the case, each SVD can be performed in unison and the compression will be the optimal one \cite{PhysRevB.62.R747}.


\subsection{\label{appendix:secImplementingTransformedOperators}Numerical implementation of the transformed bosonic operators eq. 43}
The inability of a matrix representation of $\hat{X}$ and $\hat{P}$ to obey the canonical commutation relation is easily seen by taking the trace:
\begin{equation}
    \text{Tr}([X,P]) = 0 \neq i\hbar\text{Tr}(\mathbbm{1})
\end{equation}
In the SQHO basis the "error" will accumulate near the point of truncation:
\begin{equation}
    [X,P] \doteq i\hbar
    \begin{pmatrix}
        1 & 0 \\
        0 & \ddots & \ddots \\
        & \ddots &  1 & 0 \\
        & & 0 & 1-D \\
    \end{pmatrix}
\end{equation}
Therefore, if we rely on matrix multiplication to construct the matrix representation of eq. 43 we should be wary of this defect.

From eq. 43 we see that the sub/super-diagonal matrices $a$ and $a^\dagger$ only appears quadratically. The Hamiltonian eq. \ref{appendix:eqNonGaussianHamiltonian} is also only quadratic in $X$ or $P$ such that $a$ and $a^\dagger$ only appears to the fourth power in any computation. Therefore, we can implement a matrix representation of eq. 43 simply by initializing a matrix representation of dimension $D+4$, construct the necessary Hamiltonian terms of the MPO through matrix multiplication and then truncating the matrix representations from $D+4\rightarrow D$, thereby discarding the faulty entries.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{new_figs/Example_BasisChange.pdf}
    \caption{\label{appendix:figExampleBasisChange}Absolute value of the entries of the matrices $U_{nm}^{(i)}$ used to transform the variational state from the optimized local basis $|m_i\rangle$ to the Fock basis $|n_i\rangle$: $U_{nm}^{(i)} = \langle n_i|\mathcal{U}^{(i)}|m_i\rangle$
    This example is taken from one of the results in fig. 6 with a large effective cutoff.
    }
\end{figure}

\subsection{\label{appendix:secLBO}Unifying Parameterized- and Linear Basis Optimization}
Presented in figure \ref{appendix:eqLBO} is the result of fig. 7 with the simulations of the non Gaussian experiments subjected to a round of Local Basis Optimization similar to the approach of Ref. \cite{PhysRevLett.108.160401}.
Specifically, starting from the MPS with physical dimension $d$ (namely those that produced the results corresponding to the filled dots), the linear isometry:
\begin{equation}
\adjincludegraphics[valign=c,width=0.08\linewidth]{new_figs/PurpleIsometry.png} = 
    \begin{pmatrix}
        \mathbbm{1}_{d\times d} \\
        \pmb{0}_{(D-d)\times d}
    \end{pmatrix}_{ji}
\label{appendix:eqLBO}
\end{equation}
\begin{figure}
    \centering
    \includegraphics[width=0.25\linewidth]{MPS_figs/IsometryEffectiveHamiltonian.png}
    \caption{\centering Effective Hamiltonian for isometries.}
    \label{appendix:figEffHamilIsometry}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.55\linewidth]{new_figs/Comparison_GS_pLBO_andLBO.pdf}
    \caption{\label{appendix:figLBO}The results of this figure indicates how well the parameterized local basis optimization approach can account for any variance in the basis used for computation. The variational states that correspond to the filled dots have been subjected to a single sweep of standard local basis optimization and a subsequent DMRG optimization of the corresponding MPS in the optimized basis. The obtained and improved results, after such an optimization procedure, are shown by unfilled dots. As seen, the pLBO already accounts for a lot of the variation and the gain from LBO is smaller than for the Fock-basis.}
\end{figure}
is applied to each leg, effectively increasing the physical dimension from $d$ to $D$.
The isometries are optimized similar to how the MPS is optimized in DMRG. 
Starting from e.g. the left, an effective Hamiltonian is defined for the left-most isometry, as seen in fig. \ref{appendix:figEffHamilIsometry}.
To optimize it, is to replace it with the lowest energy state of the effective Hamiltonian. 
All the isometries are optimized in a sweeping manner and after obtaining the optimal isometries the MPS is optimized with DMRG in the new $d$ dimensional basis.
The unfilled dots of fig. \ref{appendix:figLBO} correspond to the results obtained after one such sweep of updating the isometries and running DMRG.
Note that this is not the same procedure as applied in \cite{PhysRevLett.108.160401}. Furthermore, the parameterized- and standard Local Basis Optimization doesn't have to be applied separately. In fact, we suspect the optimal method would be to use L-BFGS to learn the isometry (eq. \ref{appendix:eqLBO}) simultaneously with the variational basis parameters implemented in the MPO and then use linear methods for learning the matrices of the MPS. However, this remains as a question for further studies.

\begin{widetext}
\subsection{\label{appendix:secFig4AsymptoticScaling}Fig. 4 Asymptotic Scaling}
\begin{figure*}[ht]
\centering
\subcaptionbox{\\$
\begin{aligned}
    1 - F_{\langle \psi|MPS\rangle} &\sim 0.9029 \times \varepsilon_D^{0.5347}\\
    1 - F_{\langle \psi|SVD\rangle} &\sim 0.5496  \times \varepsilon_D^{0.5201}
\end{aligned}$
}{\raisebox{+.09\height}{\includegraphics[width=0.31\textwidth,trim={0.26cm 0.28cm 0.3cm 0.25cm},clip]{new_figs/N7_FidelityVsEpsilonD_asymptotic.pdf}}}
\hfill
\subcaptionbox{\\$
\begin{aligned}
    &1 - F_{\langle \psi|MPS\rangle} \sim 0.5775 \times \varepsilon_\chi^{0.8563}\\
    &1 - F_{\langle GS|MPS\rangle} \sim 0.2721 \times \varepsilon_\chi^{0.7461}
\end{aligned}$
}{\raisebox{+.09\height}{\includegraphics[width=0.31\textwidth,trim={0.26cm 0.27cm 0.3cm 0.25cm},clip]{new_figs/N7_FidelityVsEpsilonChi3_asymptotic.pdf}}}
\hfill
\subcaptionbox{\\$
\begin{aligned}
    &1 - F_{\langle \psi|MPS\rangle} \sim 0.2901 \times \langle\mathcal{H}\rangle^{1.1827}\\
    &1 - F_{\langle GS|MPS\rangle} \sim 0.0145 \times \sqrt{\langle\mathcal{H}^2\rangle-\langle\mathcal{H}\rangle^2}^{2.1833}
\end{aligned}$}{\includegraphics[width=0.36\textwidth,trim={0.26cm 0.3cm 0.3cm 0.25cm},clip]{new_figs/PosterPlot_energyvariance4_asymptotic.pdf}}
\caption{By fitting a line to each of the datasets in all of the log-log plots we obtain the above power-law relations.
}
\end{figure*}
\newpage
\subsection{\label{appendix:secAlgebraicMPOs}Algebraic MPO construction}

The goal is to construct the MPO representation of eq. 14. Without loss of generality we can set $\pmb{\mu}=\pmb{0}=\pmb{\nu}$ because it is a simple matter to introduce them later, through a redefinition of the quadrature operators (excluding those that stem from $\pmb{\hat{\xi}}$); $\hat{X} \rightarrow \hat{X}-\mu$ and $\hat{P} \rightarrow \hat{P} - \nu$.
While it is not immediately clear how to write up the MPO for the full Hamiltonian, we begin by writing out the Hamiltonian as: 
\begin{align}
    \mathcal{H} = {\color{red} \mathcal{H}_\text{Gaussian}}
    &+ {\color{purple} \kappa\sum_i\beta_{ii}\hat{P}_i\prod_{n\neq i} \hat{X}_n
    + \kappa^2\sum_i b_{ii}\prod_{n\neq i} \hat{X}_n^2} \label{appendix:eqNonGaussianHamiltonian}\\
    &+ {\color{blue} \kappa\sum_{i\neq j} \prod_{n\neq i,j}\hat{X}_n(\gamma_{ij}\hat{X}_i^2 + b_{ij}(\hat{X}_i\hat{P}_i + \hat{P}_i\hat{X}_i)) + \kappa \text{Tr}\gamma\prod_n \hat{X}_n}
    + {\color{magenta} \kappa^2\sum_{i>j}\beta_{ij}\hat{X}_i\hat{X}_j\prod_{n\neq i,j}\hat{X}_n^2}\nonumber
\end{align}
The color coding is for more easily matching MPOs to Hamiltonian terms, also recall that this $\kappa$ is due to eq. 11, not eq. 42.
Here, $\mathcal{H}_\text{Gaussian}$ is eq. 10 and 
\begin{equation}
    \alpha_{ij} := \frac12(V^{-1})_{ij}
    \quad\quad 
    \beta_{ij} := \frac12(V^{-1})_{(N+i)(N+j)} =: 2b_{ij}
    \quad\quad
    \gamma_{ij} := \frac12(V^{-1})_{(i)(N+j)}
\end{equation}
The approach will be to write each term as an MPO and write the MPO of the full Hamiltonian as a block-diagonal MPO. This way, it is easier to derive the form of the MPO while we can still utilize the sparseness of the full MPO in the computations during optimization. %The sparseness could perhaps be utilized in a proper implementation, however, that is seemingly not straight forward in quimb/pytorch (quimb uses tensordot, and torch.tensordot is not implemented for sparse tensors).
We will for pedagogical reasons assume an odd number of modes, but it is straightforward to infer the MPOs for the case of an even number of modes. The index for the middle-most mode is denoted $N_m = (N+1)/2$.
All the MPOs will be of the form:
\begin{equation}
    \text{MPO} : \left(\prod_{s=1}^{N_m-1} L_s\right) M_{N_m}\prod_{s=N_m+1}^{N}R_s
\end{equation}
where the $L_s$', $M_{N_m}$ and $R_s$' are matrices containing operators that only act in the Hilbert space corresponding to the sub-index $s$. The idea behind every construction is to use the $L_s$' and $R_s$' to collect the relevant operator strings and then collapse the vector-matrix-vector product with the right coefficients in $M_{N_m}$, in order to yield all the terms in the Hamiltonian.
This will become clearer by considering the explicit construction of the matrices/MPO-cores in the following.

\subsubsection{{\color{red} $\mathcal{H}_\text{Gaussian}$ MPO}}
Firstly, we define the single site operator:
\begin{equation}
    \hat{S}_i = \frac{\alpha_{ii}}{2}\hat{X}^2_i + \frac{\beta_{ii}}{2}\hat{P}^2_i+\frac{\gamma_{ii}}{2}\left(\hat{X}_i\hat{P}_i+\hat{P}_i\hat{X}_i\right) - \frac{1}{2}
\end{equation}
such that the cores can be written as:
\begin{align}
    L_1 &=
    \begin{pmatrix}
        \hat{X}_1 & \hat{P}_1 & \mathbbm{1} & \hat{S}_1
    \end{pmatrix}\\
    R_N^T &= 
    \begin{pmatrix}
        \hat{X}_N & \hat{P}_N & \mathbbm{1} & \hat{S}_N
    \end{pmatrix}\\
    R_{s\neq N} &= 
    \begin{pmatrix}
        0 & 0 & & 0 & \hat{X}_s & 0 \\
        0 & 0 & \hdots & 0 & \hat{P}_s & 0 \\
        \mathbbm{1} & 0 & & 0 & 0 & 0\\
        0 & \mathbbm{1} & & 0 & 0 & 0\\
        \vdots &   & \ddots &  & \vdots & \\
        0 & 0 &  & \mathbbm{1} & 0 & 0 \\
        0 & 0 & \hdots & 0 & \mathbbm{1} & 0\\
        {\begin{aligned}&\hat{X}_s\alpha_{s(s+1)} \\&+ \hat{P}_s\gamma_{(s+1)s}\end{aligned}} & {\begin{aligned}&\hat{X}_s\gamma_{s(s+1)} \\&+ \hat{P}_s\beta_{s(s+1)}\end{aligned}} &  & {\begin{aligned}&\hat{X}_s\gamma_{sN} \\&+ \hat{P}_s\beta_{sN}\end{aligned}} & \hat{S}_s & \mathbbm{1}
    \end{pmatrix}\\
    M_{N_m} &=
    \begin{pmatrix}
        \alpha_{(N_m-1)(N_m+1)} & \gamma_{(N_m-1)(N_m+1)} &  & \alpha_{(N_m-1)N} & \gamma_{(N_m-1)N} & \alpha_{(N_m-1)N_m}\hat{X}_{N_m} + \gamma_{(N_m-1)N_m}\hat{P}_{N_m} & 0\\
        \gamma_{(N_m+1)(N_m-1)} & \beta_{(N_m-1)(N_m+1)} & \hdots & \gamma_{N(N_m-1)} & \beta_{(N_m-1)N} & \gamma_{N_m(N_m-1)}\hat{X}_{N_m} + \beta_{(N_m-1)N_m}\hat{P}_{N_m} & 0 \\
         & \vdots & \ddots &  &  & \vdots  & \\
        \alpha_{1(N_m+1)} & \gamma_{1(N_m+1)} & &\alpha_{1N} & \gamma_{1N} & \alpha_{1N_m}\hat{X}_{N_m} + \gamma_{1N_m}\hat{P}_{N_m} & 0 \\
        \gamma_{(N_m+1)1} & \beta_{1(N_m+1)} & & \gamma_{N1} & \beta_{1N} & \gamma_{N_m1}\hat{X}_{N_m} + \beta_{1N_m}\hat{P}_{N_m} & 0 \\
        {\begin{aligned}&\hat{X}_{N_m}\alpha_{N_m(N_m+1)} \\&+ \hat{P}_{N_m}\gamma_{(N_m+1)N_m}\end{aligned}} & {\begin{aligned}&\hat{X}_{N_m}\gamma_{N_m(N_m+1)} \\&+ \hat{P}_{N_m}\beta_{N_m(N_m+1)}\end{aligned}} & \hdots &
        {\begin{aligned}&\hat{X}_{N_m}\alpha_{N_mN} \\&+ \hat{P}_{N_m}\gamma_{NN_m}\end{aligned}} & {\begin{aligned}&\hat{X}_{N_m}\gamma_{N_mN} \\&+ \hat{P}_{N_m}\beta_{N_mN}\end{aligned}} &
        \hat{S}_{N_m} & \mathbbm{1}\\
        0 & 0 & & 0 & 0 & \mathbbm{1} & 0
    \end{pmatrix}
\end{align}
The $L_s$ are similar to the $R_s^T$ but,
\begin{align*}
\text{with the row:}\quad\quad\quad &\begin{pmatrix}
    {\begin{aligned}&\hat{X}_s\alpha_{s(s+1)} \\&+ \hat{P}_s\gamma_{(s+1)s}\end{aligned}} & {\begin{aligned}&\hat{X}_s\gamma_{s(s+1)} \\&+ \hat{P}_s\beta_{s(s+1)}\end{aligned}} & \hdots & {\begin{aligned}&\hat{X}_s\alpha_{s(s+1)} \\&+ \hat{P}_s\gamma_{(s+1)s}\end{aligned}}& {\begin{aligned}&\hat{X}_s\gamma_{sN} \\&+ \hat{P}_s\beta_{sN}\end{aligned}} & \hat{S}_s & \mathbbm{1}
\end{pmatrix}\\
\text{replaced by:}\quad\quad\quad &\begin{pmatrix}
    {\begin{aligned}&\hat{X}_s\alpha_{s(s-1)} \\&+ \hat{P}_s\gamma_{(s-1)s}\end{aligned}} & {\begin{aligned}&\hat{X}_s\gamma_{s(s-1)} \\&+ \hat{P}_s\beta_{s(s-1)}\end{aligned}} & \hdots & {\begin{aligned}&\hat{X}_s\alpha_{s1} \\&+ \hat{P}_s\gamma_{1s}\end{aligned}}& {\begin{aligned}&\hat{X}_s\gamma_{s1} \\&+ \hat{P}_s\beta_{s1}\end{aligned}} & \hat{S}_s & \mathbbm{1}
\end{pmatrix}
\end{align*}
\noindent\fbox{\begin{minipage}{\textwidth}
As an example, consider $N=5$:
\begin{equation}
    \includegraphics[width=1\linewidth,trim={0cm 5cm 0cm 8cm},clip]{MPS_figs/GBSMPON5.pdf}
\end{equation}
Doing the matrix multiplication gives all the terms of the Hamiltonian used for Gaussian Boson Sampling:
\begin{equation}
    {\color{red} \mathcal{H}_\text{Gaussian}} = \frac{1}{2}
    \begin{pmatrix}
        \pmb{\hat{X}} & \pmb{\hat{P}}
    \end{pmatrix}
    \left(
    \begin{array}{c|c} 
      \alpha & \gamma \\ 
      \hline 
      \gamma^T & \beta
    \end{array} 
    \right)
    \begin{pmatrix}
        \pmb{\hat{X}}\\
        \pmb{\hat{P}}
    \end{pmatrix} - \frac{N}{2} 
\end{equation}
\end{minipage}}

\subsubsection{{\color{purple} Second and third terms as MPOs} }
The MPOs of the second and third terms are more easily written up as:
\begin{align}
\sum_i\beta_{ii}\hat{P}_i\prod_{n\neq i} \hat{X}_n &= 
    \begin{pmatrix}
        \beta_{11}\hat{P}_1 & \hat{X}_1
    \end{pmatrix}
    \left(
    \prod_{n=2}^{N-1}
    \begin{pmatrix}
        \hat{X}_n & 0 \\
        \beta_{nn}\hat{P}_n & \hat{X}_n
    \end{pmatrix}
    \right)
    \begin{pmatrix}
        \hat{X}_N \\
        \beta_{NN}\hat{P}_N
    \end{pmatrix}\\
\sum_i b_{ii}\prod_{n\neq i} \hat{X}_n^2 &=
    \begin{pmatrix}
        b_{11} & \hat{X}^2_1
    \end{pmatrix}
    \left(
    \prod_{n=2}^{N-1}
    \begin{pmatrix}
        \hat{X}^2_n & 0 \\
        b_{nn} & \hat{X}^2_n
    \end{pmatrix}
    \right)
    \begin{pmatrix}
        \hat{X}^2_N \\
        b_{NN}
    \end{pmatrix}
\end{align}

\subsubsection{{\color{blue} The MPO of the fourth and fifth term}}
Now, we consider the explicit construction of the following MPO:
\begin{equation}
    \sum_{i\neq j} \prod_{n\neq i,j}\hat{X}_n(\gamma_{ij}\hat{X}_i^2 + b_{ij}(\hat{X}_i\hat{P}_i + \hat{P}_i\hat{X}_i))
    + \text{Tr}\gamma \prod_n \hat{X}_n= \left(\prod_{s=1}^{N_m-1} L_s\right) M_{N_m}\prod_{s=N_m+1}^{N}R_s
\end{equation}
To this end we define: $\Tilde{P}_n = \hat{X}_n\hat{P}_n + \hat{P}_n\hat{X}_n$ 
such that the cores can be written as:
\begin{align}
    &L_1 =
    \begin{pmatrix}
        \mathbbm{1} & \hat{X}_1 & \hat{X}_1^2 & \Tilde{P}_1
    \end{pmatrix}\\
    &R_N^T =
    \begin{pmatrix}
        \mathbbm{1} & \hat{X}_N & \hat{X}_N^2 & \Tilde{P}_N
    \end{pmatrix}\\
    &R_s = 
    \begin{pmatrix}
        \hat{X}_s & 0 & \hdots \\
        0 & \ddots &  \\
        \vdots &  & \hat{X}_s & 0 & 0 & 0\\
         & & 0 & \mathbbm{1} & 0 & 0\\
         & & 0 & \hat{X}_s & 0 & 0\\
         & & 0 & \hat{X}_s^2 & 0 & 0\\
         & & 0 & \Tilde{P}_s & 0 & 0\\
         & & 0 & 0 & \hat{X}_s& 0\\
         & & 0& 0& 0& \hat{X}_s \\
         & & & & & & \ddots\\
         & & & & & & 0 & \hat{X}_s & 0\\
         \gamma_{sN}\hat{X}_s^2+b_{sN}\Tilde{P}_{s} & \hdots& \gamma_{s(s+1)}\hat{X}_s^2 +b_{s(s+1)}\Tilde{P}_{s}& 0 &\gamma_{(s+1)s} &b_{(s+1)s} &\hdots & b_{Ns}& \hat{X}_s
    \end{pmatrix}\\
&\resizebox{1.1\hsize}{!}{$
    M_{N_m} = 
    \begin{pmatrix}
        0 & \hdots & 0 & \gamma_{N_m1}\hat{X}_{N_m}^2 + b_{N_m1}\Tilde{P}_{N_m} & \gamma_{(N_m+1)1}\hat{X}_{N_m} & b_{(N_m+1)1}\hat{X}_{N_m} & \hdots & \gamma_{N1}\hat{X}_{N_m} & b_{N1}\hat{X}_{N_m} & 0 \\
        \vdots & \ddots &  & \vdots & & & \ddots &  \\
        0 &  & 0 & \gamma_{N_m(N_m-1)}\hat{X}_{N_m}^2 + b_{N_m(N_m-1)}\Tilde{P}_{N_m} & \gamma_{(N_m+1)(N_m-1)}\hat{X}_{N_m} & b_{(N_m+1)(N_m-1)}\hat{X}_{N_m} & \hdots & \gamma_{N(N_m-1)}\hat{X}_{N_m} & b_{N(N_m-1)}\hat{X}_{N_m} & 0 \\
        \gamma_{N_mN}\hat{X}_{N_m}^2 + b_{N_mN}\Tilde{P}_{N_m} & \hdots & 
        \gamma_{N_m(N_m+1)}\hat{X}_{N_m}^2 + b_{N_m(N_m+1)}\Tilde{P}_{N_m}
        & \text{Tr}\gamma \hat{X}_{N_m} & \gamma_{(N_m+1)N_m} & b_{(N_m+1)N_m} & \hdots & \gamma_{NN_m} & b_{NN_m} & \hat{X}_{N_m} \\
        \gamma_{(N_m-1)N}\hat{X}_{N_m} & & \gamma_{(N_m-1)(N_m+1)}\hat{X}_{N_m} & \gamma_{(N_m-1)N_m} & 0 & 0 \\
        b_{(N_m-1)N}\hat{X}_{N_m} & & b_{(N_m-1)(N_m+1)}\hat{X}_{N_m} & b_{(N_m-1)N_m} & 0 & \ddots \\
        \vdots & \ddots & \vdots \\
        \gamma_{1N}\hat{X}_{N_m} & & \gamma_{1(N_m+1)}\hat{X}_{N_m} & \gamma_{1N_m} \\
        b_{1N}\hat{X}_{N_m} & & b_{1(N_m+1)}\hat{X}_{N_m} & b_{1N_m} & & &  & &\ddots &0\\
        0 & \hdots & 0 & \hat{X}_{N_m} & & & && 0& 0
    \end{pmatrix}$}
\end{align}
The $L_s$ are similar to the $R_s^T$ but,
\begin{align*}
\text{with the row:}\quad\quad\quad &\begin{pmatrix}
    \gamma_{sN}\hat{X}_s^2+b_{sN}\Tilde{P}_{s}& \hdots& \gamma_{s(s+1)}\hat{X}_s^2+b_{s(s+1)}\Tilde{P}_{s}& 0 &\gamma_{(s+1)s} &b_{(s+1)s} &\hdots & b_{Ns}& \hat{X}_s
\end{pmatrix}\\
\text{replaced by:}\quad\quad\quad &\begin{pmatrix}
    \gamma_{s1}\hat{X}_s^2++b_{s1}\Tilde{P}_{s}& \hdots& \gamma_{s(s-1)}\hat{X}_s^2++b_{s(s-1)}\Tilde{P}_{s}& 0 &\gamma_{(s-1)s} &b_{(s-1)s} &\hdots & b_{1s}& \hat{X}_s
\end{pmatrix}
\end{align*}

\subsubsection{{\color{magenta} The MPO for the last term}}
Again, we write the MPO as:
\begin{equation}
    \sum_{i>j}\beta_{ij}\hat{X}_i\hat{X}_j\prod_{n\neq i,j}\hat{X}_n^2 = \left(\prod_{s=1}^{N_m-1} L_s\right) M_{N_m}\prod_{s=N_m+1}^{N}R_s
\end{equation}
this time with: 
\begin{align}
    &L_1 =
    \begin{pmatrix}
        \hat{X}_1^2 & \hat{X}_1
    \end{pmatrix}\\
    &R_N^T =
    \begin{pmatrix}
        \hat{X}_N^2 & \hat{X}_N
    \end{pmatrix}\\
    &R_s = 
    \begin{pmatrix}
        \hat{X}_s^2 & 0 \\
        \hat{X}_s & 0 \\
        0 & \hat{X}_s^2  \\
        & & \ddots \\
        & & &\hat{X}_s^2 \\
        0 & \beta_{(s+1)s}\hat{X}_s & \hdots & \beta_{Ns}\hat{X}_s & \hat{X}_s^2
    \end{pmatrix}\\
    &M_{N_m} = 
    \begin{pmatrix}
        0 & \beta_{(N_m+1)N_m}\hat{X}_{N_m} & \hdots & \beta_{NN_m}\hat{X}_{N_m} & \hat{X}_{N_m}^2 \\
        \beta_{N_m(N_m-1)}\hat{X}_{N_m} & \beta_{(N_m+1)(N_m-1)}\hat{X}_{N_m}^2 & \hdots & \beta_{N(N_m-1)}\hat{X}_{N_m}^2 & 0 \\
        \vdots  & \vdots & \ddots &\vdots & \vdots \\
        \beta_{N_m1}\hat{X}_{N_m} & \beta_{(N_m+1)1}\hat{X}_{N_m}^2 & \hdots & \beta_{N1}\hat{X}_{N_m}^2 & 0 \\
        \hat{X}_{N_m}^2 & 0&\hdots & 0& 0
    \end{pmatrix}
\end{align}
The $L_s$ are similar to the $R_s^T$ but,
\begin{align*}
\text{with the row:}\quad\quad\quad &\begin{pmatrix}
    0 & \beta_{(s+1)s}\hat{X}_s & \hdots & \beta_{Ns}\hat{X}_s & \hat{X}_s^2
\end{pmatrix}\\
\text{replaced by:}\quad\quad\quad &\begin{pmatrix}
    0 & \beta_{s(s-1)}\hat{X}_s & \hdots & \beta_{s1}\hat{X}_s & \hat{X}_s^2
\end{pmatrix}
\end{align*}
\end{widetext}


